MeshLRM: Large Reconstruction Model for High-Quality Meshes

We propose MeshLRM, a novel LRM-based approach that can reconstruct a high-quality mesh from merely four input images in less than one second. Different from previous large reconstruction models (LRMs) that focus on NeRF-based reconstruction, MeshLRM incorporates differentiable mesh extraction and rendering within the LRM framework. This allows for end-to-end mesh reconstruction by fine-tuning a pre-trained NeRF LRM with mesh rendering. Moreover, we improve the LRM architecture by simplifying several complex designs in previous LRMs. MeshLRM's NeRF initialization is sequentially trained with low- and high-resolution images; this new LRM training strategy enables significantly faster convergence and thereby leads to better quality with less compute. Our approach achieves state-of-the-art mesh reconstruction from sparse-view inputs and also allows for many downstream applications, including text-to-3D and single-image-to-3D generation. Project page: https://sarahweiii.github.io/meshlrm/

==> tables/ablate_ft.tex <==
% \begin{table}[h]
% \centering
% \caption{The performance gap when transferring the MesnLRM (NeRF) to surface rendering using post-processing marching cubes and the effectiveness of our fine-tuning stage with differentiable marching cubes and rasterization.} 
% \label{tab:ablate_ft}
% \begin{tabular}{l|cccc} 
% \toprule
%                      & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & CD$\downarrow$    \\ 
% \midrule
% MeshLRM (NeRF)         & \textbf{28.13} & 0.923 & 0.093 &     - \\
% MeshLRM (NeRF)+MC   & 25.48 & 0.903 & 0.087 & 3.26  \\
% MeshLRM               & 27.93 & \textbf{0.925} & \textbf{0.070} & \textbf{2.68}  \\
% \bottomrule
% \end{tabular}
% \end{table}
